Robust Prompt Optimization for Large Language Models Against Distribution Shifts

Large Language Model (LLM) has demonstrated significant ability in various Natural Language Processing tasks. However, their effectiveness is highly dependent on the phrasing of the task prompt, leading to research on automatic prompt optimization using labeled task data. We reveal that these prompt optimization techniques are vulnerable to distribution shifts such as subpopulation shifts, which are common for LLMs in real-world scenarios such as customer reviews analysis. In this light, we propose a new problem of robust prompt optimization for LLMs against distribution shifts, which requires the prompt optimized over the labeled source group can simultaneously generalize to an unlabeled target group. To solve this problem, we propose Generalized Prompt Optimization framework, which incorporates the unlabeled data from the target group into prompt optimization. Extensive experimental results demonstrate the effectiveness of the proposed framework with significant performance improvement on the target group and comparable performance on the source group.

==> emnlp2023-latex/2_analysis_0620.tex <==
% TODO:
% problem formulation和后面的符号或许需要改.

\section{Preliminary Experiments} \label{sec:preliminart_experiments}

In this section, we identify the generalization issue of prompt optimization with distribution shifts through experimental results, and perform analysis regarding the generalization ability of different source groups to optimize prompts. 
We introduce the problem formulation, the dataset selection, the baseline method, the implementation detail and the experimental results, respectively. 
% 老板comments 7: 需添加insights。
% We select 16 datasets spanning across 6 tasks, and regard different datasets of the same task as different groups with distribution shift. We use a LLM-based instruction optimization method \textit{APE}, and generate the optimized prompt for each data group. 
% For each group, we compare the performance of the optimized prompt on this group, and the optimized prompt generalized from another group to observe the generalization performance gap. 


\subsection{Problem Formulation} \label{sec:preliminart_experiments_problem_definition}
The prompt optimization aims to find the best prompt $\textbf{p}$ that LLM can successfully map the concatenation of $\textbf{p}$ and task input $\textbf{x}$ into the corresponding output $\textbf{y}$, where $\textbf{x}, \textbf{y}$ and $\textbf{p}$ are all word sequences. 
Suppose that the task data $(\textbf{x}, \textbf{y})$ follows a distribution $D$, the goal is to obtain $\textbf{p}^o = argmax_{\textbf{p} \in \mathcal{Z}} r(LLM(\textbf{p}, \textbf{x}), \textbf{y}), (\textbf{x}, \textbf{y}) \sim D$. $\mathcal{Z}$ denotes the prompt space, \eg the space of word sequences, and $r$ is the evaluation metric between the LLM output and the ground truth output $\textbf{y}$, \eg Accuracy.
% 不写loss，不写1/N； 

We consider the prompt generalization setting of two data groups, the source group data $(\textbf{x}_{s}, \textbf{y}_{s})$ following distribution $D_{s}$, and the target group data $(\textbf{x}_t, \textbf{y}_t)$ following a different distribution $D_{t}$. We intend to find whether the optimized prompt of the source group $\textbf{p}_s^o = \arg\max_{\textbf{p} \in \mathcal{Z}} r(LLM(\textbf{p}, \textbf{x}_s), \textbf{y}_s), (\textbf{x}_s, \textbf{y}_s) \sim D_s$ can have comparable target group performance as the optimized prompt on the target group $\textbf{p}_t^o = argmax_{\textbf{p} \in \mathcal{Z}} r(LLM(\textbf{p}, \textbf{x}_t), \textbf{y}_t), (\textbf{x}_t, \textbf{y}_t) \sim D_t$. 

% 不指定seen unseen的分布关系。不写loss, 写成reward/acc, 不写1/N，

\subsection{Datasets}
We select 16 datasets across 6 popular NLP tasks. 
To create distribution shifts between datasets, we select datasets following recent out-of-distribution (OOD) and adversarial robustness research \cite{yang2022glue}, and datasets with different background information. We regard each dataset as a group, where between the groups exist distribution shifts \cite{arora2021types}. 
% Our criteria for dataset selection follow recent studies on out-of-distribution (OOD) generalization \cite{yang2022glue, arora2021types}. We select datasets that are created as OOD robustness evaluation, or datasets of different domains, \eg different topics. 
For sentiment analysis task, we adopt Yelp \cite{zhang2015character}, Flipkart \cite{flipkart}, IMDB \cite{maas-EtAl:2011:ACL-HLT2011} and Amazon \cite{zhang2015character} of different topics. 
For natural language inference task, we utilize MNLI \cite{williams2018broad}, and ANLI \cite{nie2020adversarial} which is an adversarial dataset for MNLI. 
For textual entailment task, we use RTE \cite{wang2018glue} and its OOD dataset HANS \cite{mccoy2019right}. 
For multi-choice commonsense QA task, we use SocialIQA \cite{sap2019socialiqa}, PIQA \cite{bisk2020piqa}, and OpenbookQA \cite{mihaylov2018can}, which focus on different types of commonsense knowledge. 
For dialog response selection task, we use DSTC7 \cite{gunasekara2019dstc7}, Ubuntu Dialog \cite{lowe2015ubuntu}, and MuTual \cite{cui2020mutual}, which are about different dialog topics. 
We also use two data splits of the numerical QA task DROP \cite{dua2019drop} with different answer types as two groups:  numerical value or text spans as answer. All tasks are classification tasks except for DROP. 
Table~\ref{} shows a summary for all datasets.
% LLM如果已经见过了怎么办？任务太简单了，不清楚新任务上的performance怎么办？

\subsection{Baseline Method}
% We adopt \textit{APE} \cite{zhou2023large} a gradient-free prompt optimization method for LLM, as our baseline method for prompt generalization analysis. 
We adopt APE \cite{zhou2023large}, an effective gradient-free LLM prompt optimization method, as our baseline method for prompt generalization analysis. 
% 选择的原因
APE can obtain prompts of high quality and easily surpass human-written prompts on NLP tasks. 
APE first leverages LLM to generate various candidate prompts by providing it with input-output examples, then performs prompt evaluation and Monte Carlo search to select and refine the prompt with the best validation performance. 
To clearly show the effect of prompts, we currently experiment with the zero-shot setting. 
% largely outperforms recent RL-based method on LLM \cite{diao2022black, zhang2023tempera}. 
% designed for black-box LLM, which does not require any knowledge on the parameter detail of LLM. Due to the strong generation ability of LLM, even without access to parameter detail, APE can generate instructions of high quality which are comparable to and often surpass human-written instructions. We believe this method will have wider application potential. 
% Besides, compared to recent Reinforcement Learning based method \cite{diao2022black, zhang2023tempera}, instructions obtained from APE is highly cost-effective and interpretable. Also, \citeauthor{pryzant2023automatic} show that APE largely outperforms RL-based methods. 
% Figure xx briefly illustrate the process of APE. 
% APE split the training examples into $M \times N$ splits, and feed each split of $N$ examples into LLM with a meta instruction to generate an instruction. After generating $M$ instructions, the instructions are tested with validation data and ranked the validation performance, and the instruction with optimal validation performance is identified for testing. 
For backbone LLM, we use a fixed version of ChatGPT \cite{ouyang2022training}, \textit{gpt-3.5-turbo-0301}, which is one of the most powerful LLM excelled at language understanding and generation, by calling the OpenAI API\footnote{\url{https://chat.openai.com/}}. 

\subsection{Implementation Detail}
% 参数设定。 
For each dataset, we use the training set to split into training and validation set, and randomly select 150 instances from the original validation set as our test set as sometimes the labels for the original test set are not available. 
Given the randomness of the backbone LLM, we set the temperature of LLM as 0, top-p as 1.0, and run 5 times with different random seed to obtain the averaged results. 
Following the setting of APE, for each run, we randomly sample 36-shot training and 36-shot validation data for prompt optimization. 
% test the obtained optimized prompt on the test data to report the averaged result. 
The detailed data splits and parameter setting can be found in Appendix~\ref{}. 
% The detailed parameter selection and setting are listed in the Appendix. 
% evaluation metric
For all classification tasks, we use accuracy as the evaluation metric. For DROP, we utilize its standard evaluation metric of F1. 

\subsection{Experimental Results}
\paragraph{Demonstration of Generalization Performance Gap.}
% We intend to observe whether the prompt optimized in the source group can still effectively generalize to the target group, by comparing the target group performance on the prompts optimized on the source and target groups, respectively. 
We treat each pair of groups of the same task as the source and target groups. 
%The results are shown in Tables~\ref{tab:analysis_no_gap} and \ref{tab:analysis_with_gap}, where each table shows the groups for one task. 
Table~\ref{tab:analysis_no_gap} shows the tasks that no large generalization gap exists, and Table~\ref{tab:analysis_with_gap} shows other tasks where large gaps (>8.0) exist between some groups. 
The row headers refer to the source group where the prompts are optimized on. The column headers refer to the target group where the optimized prompts are tested on. The generalization performance gap is observed by comparing the different values of the same column. 


\begin{table}[h]
    \begin{subtable}[h]{0.5\textwidth}
        \centering
        \resizebox{0.7\textwidth}{!}{
        \centering
\begin{tabular}{l|l|l}
\toprule
\backslashbox{Source}{Target} & MNLI       & ANLI   \\
\midrule
MNLI & 73.4 $\pm$ 1.0 & 45.4 $\pm$ 1.9 \\
ANLI & 73.3 $\pm$ 1.3 & 46.0 $\pm$ 1.5 \\ 
\bottomrule
\end{tabular} 
       }
       \caption{Natural language inference }
       \label{tab:analysis_nli}
    \end{subtable}
    %\hfill
    \\
    \begin{subtable}[h]{0.5\textwidth}
        \centering
        \resizebox{0.7\textwidth}{!}{
\begin{tabular}{l|l|l}
\toprule
\backslashbox{Source}{Target}& RTE        & HANS       \\
\midrule
RTE  & 78.3 $\pm$ 0.8 & 67.2 $\pm$ 1.1 \\
HANS & 79.0 $\pm$ 0.8 & 68.4 $\pm$ 1.8 \\ 
\bottomrule
\end{tabular} 
    }
       \caption{Textual entailment }
       \label{tab:analysis_rte}
    \end{subtable}
    % \hfill
    \\
    \begin{subtable}[h]{0.5\textwidth}
        \centering
        \resizebox{\textwidth}{!}{
\begin{tabular}{l|l|l|l}
\toprule
\backslashbox{Source}{Target} & DSTC7               & Ubuntu Dialog       & MuTual              \\
\midrule
DSTC7         & 58.4 $\pm$ 0.8 & 78.9 $\pm$ 0.3 & 74.2 $\pm$ 2.2          \\
Ubuntu Dialog & 56.9 $\pm$ 1.3          & 78.7 $\pm$ 0.5          & 74.4 $\pm$ 2.1          \\
MuTual        & 52.2 $\pm$ 4.4          & 74.7 $\pm$ 6.0          & 76.7 $\pm$ 3.4 \\ 
\bottomrule
\end{tabular}
        }
        \caption{Dialog}
        \label{tab:analysis_mcdialog}
     \end{subtable}
     \caption{Results for tasks without large generalization performance gap across groups. 
     % The row headers and column headers indicate the source and target groups, respectively. 
     } 
     \label{tab:analysis_no_gap}
\end{table}

\begin{table}[h]
    \begin{subtable}[t]{0.5\textwidth}
        \centering
        \resizebox{\textwidth}{!}{
\begin{tabular}{l|l|l|l|l}
\toprule
\backslashbox{Source}{Target} & Yelp                & Flipkart            & IMDB                & Amazon      \\ 
\midrule
Yelp     & \textbf{79.7 $\pm$ 0.7} & 78.4 $\pm$ 1.9          & 87.1 $\pm$ 1.9          & 88.4 $\pm$ 1.9  \\
Flipkart & 69.1 $\pm$ 8.7          & \textbf{85.1 $\pm$ 2.9} & 85.2 $\pm$ 9.4          & 85.9 $\pm$ 12.5 \\
IMDB     & 71.1 $\pm$ 8.2          & 76.9 $\pm$ 13.4         & \textbf{91.9 $\pm$ 0.9} & 90.4 $\pm$ 5.2  \\
Amazon   & 75.5 $\pm$ 1.5          & \textbf{85.6 $\pm$ 2.1} & \textbf{91.5 $\pm$ 0.8} & \textbf{93.5 $\pm$ 1.4}  \\ 
\bottomrule
\end{tabular}
       }
       \caption{Sentiment analysis }
       \label{tab:analysis_sa}
    \end{subtable}
    %\hfill
    \\
    \begin{subtable}[t]{0.5\textwidth}
        \centering
        \resizebox{\textwidth}{!}{
\begin{tabular}{l|l|l|l}
\toprule
\backslashbox{Source}{Target}  & SocialIQA           & PIQA                & OpenbookQA          \\
\midrule
SocialIQA  & 75.6 $\pm$ 1.4 & 82.0 $\pm$ 6.0          & 71.2 $\pm$ 5.2          \\
PIQA       & 68.9 $\pm$ 6.9          & 83.6 $\pm$ 2.9 & 69.2 $\pm$ 5.1          \\
OpenbookQA & \textbf{79.9 $\pm$ 1.0}  & \textbf{84.5 $\pm$ 1.6}  & \textbf{80.1 $\pm$ 2.4} \\ 
\bottomrule
\end{tabular}
    }
       \caption{Commonsense QA}
       \label{tab:analysis_mcqa}
    \end{subtable}
    %\hfill
    \\
    \begin{subtable}[t]{0.5\textwidth}
        \centering
        \resizebox{0.7\textwidth}{!}{
\begin{tabular}{l|l|l}
\toprule
\backslashbox{Source}{Target} & Number     & Spans      \\
\midrule
Number & 51.9 $\pm$ 2.8 & 20.1 $\pm$ 1.3 \\
Spans  & \textbf{57.7 $\pm$ 2.9} & \textbf{63.1 $\pm$ 2.2} \\
\bottomrule
\end{tabular}
        }
        \caption{DROP}
        \label{tab:analysis_drop}
     \end{subtable}
     \caption{Results for tasks with significant generalization performance gap across groups. Bold font indicates the largest value for each column. }
     \label{tab:analysis_with_gap}
\end{table}

From the tables, we can observe:
1) The generalization performance gap may not exist for previously studied OOD and adversarial groups, including the groups of the natural language inference and the textual entailment tasks, which is attributed to the strong generalization ability of LLM. 
2) However, under some distribution shifts, \eg 

the sentiment analysis datasets and the commonsense QA datasets with different topics, \eg
Flipkart and Yelp, PIQA and OpenbookQA, and the DROP groups with different answer types, 
there still exist significant generalization performance gaps, demonstrating the existence of the generalization issue of prompt optimization. 
% Moreover, the generalization performance sometimes tends to have much larger variance than the performance of the optimized prompts of the target group, showing larger instability of the generalized instructions. 
3) Surprisingly, the prompt optimized from the source group does not always perform worse than the prompt optimized on the target group. For commonsense QA task, the generalized prompt from OpenbookQA performs even better than the optimized prompt for SocialIQA. Also, for DROP, the generalized prompt from Spans perform better than the optimized prompt for Number. 
% We conjecture that this phenomenon is related to the larger diversity of the source group leading to more robust prompts. 


% case study?
\paragraph{Exploration on the Relevant Factors of Prompt Robustness.}
Based on the above observations, we further explore two research questions. 

\textbf{Q1}: \textit{Why do the prompts optimized on different source groups have different generalization performance on a target group? }
\textbf{Q2}: \textit{Why in some cases the prompts generalized from the source group performs even better than the optimized prompt on the target group?}
% 还需要再想一下

To address Q1, we conjecture that the better generalization performance is related to a smaller distribution shifts between the source and target groups. 
Therefore, we examine two metrics to measure the distribution shifts: the label distribution shift which is the KL divergence between the label distributions of the two groups for the classification tasks, and the input similarity which quantifies the n-gram similarity of the input corpuses of the two groups. 
The detailed implementation is illustrated in Appendix~\ref{}. 
We show the results of the sentiment analysis task as an example in Table~\ref{tab:metrics_sa}. 
We can observe that the smallest label distribution shifts and the largest input similarity generally coincide with the best generalization performance on each target group, thus the two metrics may empirically correlate to the generalization performance. However, the two metrics are not perfectly effective for other tasks (\cf Appendix), and also they cannot be compared across target groups nor across tasks. Therefore, Q1 is still a challenging research question that requires further exploration. 

\begin{table}[h]
    \begin{subtable}[t]{0.5\textwidth}
        \centering
        \resizebox{0.8\textwidth}{!}{
\begin{tabular}{l|llll}
\toprule
\backslashbox{Source}{Target} & Yelp     & Flipkart      & IMDB       & Amazon     \\
\midrule
Yelp     & -             & 0.33          & 1.62       & 1.62       \\
Flipkart & 0.30          & -             & 0.57       & 0.56       \\
IMDB     & \textbf{0.25} & 0.29          & -          & \textbf{0} \\
Amazon   & \textbf{0.25} & \textbf{0.27} & \textbf{0} & -          \\
\bottomrule
\end{tabular}
       }
       \caption{Label distribution shifts. Smaller value indicates less distribution shift. }
       \label{tab:metric_sa_label_shift}
    \end{subtable}
    % \hfill 
    \\
    \begin{subtable}[t]{0.5\textwidth}
        \centering
        \resizebox{0.8\textwidth}{!}{
\begin{tabular}{l|llll}
\toprule
\backslashbox{Source}{Target} & Yelp    & Flipkart      & IMDB          & Amazon        \\
\midrule
Yelp     & -             & 0.65          & 0.73          & 0.76          \\
Flipkart & 0.59          & -             & 0.55          & 0.63          \\
IMDB     & 0.70          & 0.63          & -             & \textbf{0.81} \\
Amazon   & \textbf{0.71} & \textbf{0.70} & \textbf{0.78} & -   \\
\bottomrule
\end{tabular}
    }
       \caption{Input similarity. Larger value indicates less distribution shift. }
       \label{tab:metric_sa_input_sim}
    \end{subtable}
    % \hfill
    \\
     \caption{Results for (a) label distribution shifts (b) input similarity of the sentiment analysis datasets. Bold font indicates the least distribution shift for each column. }
     \label{tab:metrics_sa}
\end{table}

\begin{table}[h]
    \begin{subtable}[t]{0.5\textwidth}
        \centering
        \resizebox{0.8\textwidth}{!}{
\begin{tabular}{llll}
\toprule
  & SocialIQA & PIQA & OpenbookQA    \\
\midrule
word 1-gram  & 0.43      & 0.51 & \textbf{0.58} \\
char 4-gram  & 0.50      & 0.60 & \textbf{0.65} \\
\bottomrule
\end{tabular}
       }
       \caption{The n-gram diversity.}
       \label{tab:metric_mcqa_1}
    \end{subtable}
    %\hfill
    \\
    \begin{subtable}[t]{0.5\textwidth}
        \centering
        \resizebox{0.8\textwidth}{!}{
\begin{tabular}{l|lll}
\toprule
\backslashbox{Source}{Target} & SocialIQA     & PIQA          & OpenbookQA    \\
\midrule
SocialIQA  & -             & 0.39          & 0.38          \\
PIQA       & 0.47          & -             & \textbf{0.46}         \\
OpenbookQA & \textbf{0.51} & \textbf{0.52} & -             \\
\bottomrule
\end{tabular}
    }
       \caption{The word 1-gram coverage ratio between groups. }
       \label{tab:metric_mcqa_2}
    \end{subtable}
    %\hfill
    \\
    \begin{subtable}[t]{0.5\textwidth}
        \centering
        \resizebox{0.8\textwidth}{!}{
\begin{tabular}{l|lll}
\toprule
\backslashbox{Source}{Target} & SocialIQA     & PIQA          & OpenbookQA    \\
\midrule
SocialIQA  & -             & 0.51          & 0.51          \\
PIQA       & 0.60          & -             & \textbf{0.58}          \\
OpenbookQA & \textbf{0.66} & \textbf{0.64} & -             \\
\bottomrule
\end{tabular}
        }
        \caption{The char 4-gram coverage ratio between groups. }
        \label{tab:metric_mcqa_3}
     \end{subtable}
     \caption{Evaluation on (a) the n-gram diversity and (b) word 1-gram coverage ratio (c) char 4-gram coverage ratio of commonsense QA datasets to study the even higher generalization performance. Bold font indicates the largest value for each column. }
     \label{tab:metric_mcqa_q2}
     % \vspace{-20pt}
\end{table}

% The label distribution shift quantifies the divergence of the label distributions between two groups for classification tasks, calculated by the KL divergence of their label distributions, $D_{KL} = \sum_{y \in \mathcal{Y}} P_s(y)log(\frac{P_s(y)}{P_t(y)})$, where $\mathcal{Y}$ is the label space of the task, and $P_s (y)$ and $P_t(y)$ denote the probability of the label $y$ in the source and target groups, respectively. 

% The input similarity quantifies the n-gram similarity of the input corpuses of the two groups.Suppose that the inputs of the source and the target groups are denoted as $x_s = \{x_{s_1}, ..., x_{s_N}\}$ and $x_t = \{x_{t_1}, ..., x_{t_N}\}$, we calculate the Spearman's rank order correlation between the bag-of-word vectors of $x_s$ and $x_t$, $\rho = \frac{cov(V_s, V_t)}{\delta(V_s)\delta(V_t)}$, where $V_s$ and $V_t$ denotes the ranked bag-of-word vectors of $x_s$ and $x_t$ on the vocabulary of $x_t$. 

% We choose two representative tasks with generalization performance gap: sentiment analysis and multi-choice commonsense QA, and one task without generalization performance gap: the dialog response selection, to evaluate the correlation between the proposed metrics and the generalization performance. For the same task, we sample each group a fixed number of instances to calculate the metrics. 


%The evaluation for label distribution shift is shown in Table~\ref{tab:metrics_label_shift}. We can observe that for sentiment analysis, the smallest label distribution shifts generally coincide with the best generalization performance of different source groups. 
%However, this does not hold for multi-choice commonsense QA, which is probably due to the too large difference in the label distribution. 
%The zero shift of dialog response selection task also coheres with the small generalization performance difference. The observation shows that the label distribution shift is weakly correlated to the generalization performance, yet cannot stably indicate the result.
%The evaluation for input similarity is shown in Table~\ref{tab:metrics_input_similarity}. We can observe that for sentiment analysis and multi-choice commonsense QA, the largest input similarities generally coincide with the best generalization performance for each group, and the close input similarity for dialog response selection also related to the tiny difference in generalization performance. 
%Nevertheless, we find that these metrics cannot be compared across target groups nor across tasks, \ie a smaller input similarity with another target group cannot indicate worse generalization performance on the other group. Therefore, Q1 is still a challenging research question that requires further exploration. 


For Q2, we conjecture that the outstanding generalization performance is caused by obtaining the prompt from a source group with large diversity, and sufficient inclusion of the patterns in the target group. % 不仅是相似，而且是单向的包含。
Therefore, we make a first attempt by evaluating the percentage of unique n-grams, and the percentage of target group n-grams that are included in the source group for the commonsense QA task, as shown in Table~\ref{tab:metric_mcqa_q2}. 
We can observe that according to the n-gram statistics, OpenbookQA has the most diverse input with the largest proportion of unique n-grams. Moreover, OpenbookQA has already covered a large proportion of n-grams of SocialIQA and PIQA, which may correlate to its strong generalization as shown in Table~\ref{tab:analysis_with_gap}. 
% However, due to the complexity of the inner mechanism of LLM, it is currently not possible to stably identify the phenomenon with these metrics, requiring a deeper understanding the generalization ability of LLM. 
% coverage ratio of the input corpuses of the multi-choice commonsense QA task. 
% We still sample the same amount of training instances for the three groups. Denote the sampled input corpuses for SocialIQA, PIQA and OpenbookQA as $x_1, x_2$ and $x_3$. % corpus 可以用小x吗？
%Firstly, we calculate the proportion of unique n-grams for each group against all n-grams for the three corpuses as $\text{n-grams}(x_i) / \text{n-grams}(\{x_1, x_2, x_3\}), i = 1, 2, 3$, as shown in Table~\ref{tab:metric_mcqa_1}. 
%Secondly, we think the source group that has already covered a larger proportion of n-grams of the target group may promote better generalization, and we calculate the proportion of n-gram coverage between the source and target groups as $\text{n-grams}(x_s) \cap \text{n-grams}(x_t) / \text{n-grams}(x_t)$. The results are shown in Table~\ref{tab:metric_mcqa_2} and Table~\ref{tab:metric_mcqa_3}. 



% \begin{table}[htbp!]
% \centering
% \resizebox{0.49\textwidth}{!}{
% \begin{tabular}{lll|lll}
% \toprule
%      & MNLI       & ANLI       &      & RTE        & HANS       \\
% \midrule
% MNLI & 73.4 + 1.0 & 45.4 + 1.9 & RTE  & 78.3 + 0.8 & 67.2 + 1.1 \\
% ANLI & 73.3 + 1.3 & 46.0 + 1.5 & HANS & 79.0 + 0.8 & 68.4 + 1.8 \\ 
% \bottomrule
% \end{tabular}
% }
% \caption{Results for NLI and RTE}
% \label{tab:analysis_nli_rte}
% \end{table}

% \begin{table}[htbp!]
% \centering
% \resizebox{0.49\textwidth}{!}{
% \begin{tabular}{llll}
% \toprule
%               & DSTC7               & Ubuntu Dialog       & MuTual              \\
% \midrule
% DSTC7         & \textbf{58.4 $\pm$ 0.8} & \textbf{78.9 $\pm$ 0.3} & 74.2 $\pm$ 2.2          \\
% Ubuntu Dialog & 56.9 $\pm$ 1.3          & 78.7 $\pm$ 0.5          & 74.4 $\pm$ 2.1          \\
% MuTual        & 52.2 $\pm$ 4.4          & 74.7 $\pm$ 6.0          & \textbf{76.7 $\pm$ 3.4} \\ 
% \bottomrule
% \end{tabular}
% }
% \caption{Results for dialog response selection}
% \label{tab:analysis_mcdialog}
% \end{table}

% \begin{table}[htbp!]
% %\setlength{\abovecaptionskip}{0.05cm}
% %\setlength{\belowcaptionskip}{-0.45cm}
% \centering
% \resizebox{0.49\textwidth}{!}{

% \begin{tabular}{lllll}
% \toprule
%          & Yelp                & Flipkart            & IMDB                & Amazon      \\ 
% \midrule
% Yelp     & \textbf{79.7 $\pm$ 0.7} & 78.4 $\pm$ 1.9          & 87.1 $\pm$ 1.9          & 88.4 $\pm$ 1.9  \\
% Flipkart & 69.1 $\pm$ 8.7          & \textbf{85.1 $\pm$ 2.9} & 85.2 $\pm$ 9.4          & 85.9 $\pm$ 12.5 \\
% IMDB     & 71.1 $\pm$ 8.2          & 76.9 $\pm$ 13.4         & \textbf{91.9 $\pm$ 0.9} & 90.4 $\pm$ 5.2  \\
% Amazon   & 75.5 $\pm$ 1.5          & \textbf{85.6 $\pm$ 2.1} & \textbf{91.5 $\pm$ 0.8} & \textbf{93.5 $\pm$ 1.4}  \\ 
% \bottomrule
% \end{tabular}

% }
% \caption{Results for Sentiment Analysis}
% \label{tab:analysis_sa}
% \end{table}


% \begin{table}[]
% \centering
% \resizebox{0.3\textwidth}{!}{
% \begin{tabular}{lll}
% \toprule
%        & number     & spans      \\
% \midrule
% number & 51.9 $\pm$ 2.8 & 20.1 $\pm$ 1.3 \\
% spans  & \textbf{57.7 $\pm$ 2.9} & \textbf{63.1 $\pm$ 2.2} \\
% \bottomrule
% \end{tabular}
% }
% \caption{Results for DROP}
% \label{tab:analysis_drop}
% \end{table}


% \begin{table}[]
% \centering
% \resizebox{0.49\textwidth}{!}{
% \begin{tabular}{llll}
% \toprule
%            & SocialIQA           & PIQA                & OpenbookQA          \\
% \midrule
% SocialIQA  & \textbf{75.6 $\pm$ 1.4} & 82.0 $\pm$ 6.0          & 71.2 $\pm$ 5.2          \\
% PIQA       & 68.9 $\pm$ 6.9          & \textbf{83.6 $\pm$ 2.9} & 69.2 $\pm$ 5.1          \\
% OpenbookQA & 79.9 $\pm$ 1.0          & 84.5 $\pm$ 1.6          & \textbf{80.1 $\pm$ 2.4} \\ 
% \bottomrule
% \end{tabular}
% }
% \caption{Results for commonsense MCQA}
% \label{tab:analysis_commonsense}
% \end{table}







% \begin{table}[]
% \centering
% \resizebox{0.49\textwidth}{!}{
% \begin{tabular}{lllll}
% \toprule
%          & Yelp          & Flipkart      & IMDB          & Amazon        \\
% \midrule
% Yelp     & -             & 0.65          & 0.73          & 0.76          \\
% Flipkart & 0.59          & -             & 0.55          & 0.63          \\
% IMDB     & 0.70          & 0.63          & -             & \textbf{0.81} \\
% Amazon   & \textbf{0.71} & \textbf{0.70} & \textbf{0.78} & -   \\
% \bottomrule
% \end{tabular}
% }
% \caption{Results for input similarity (larger indicates more similar and better generalization performance)}
% \label{tab:metric_sa_input_similarity}
% \end{table}

% \begin{table}[]
% \centering
% \resizebox{0.49\textwidth}{!}{
% \begin{tabular}{llll}
% \toprule
%            & SocialIQA     & PIQA          & OpenbookQA    \\
% \midrule
% SocialIQA  & -             & 0.59          & 0.62          \\
% PIQA       & 0.57          & -             & \textbf{0.69} \\
% OpenbookQA & \textbf{0.61} & \textbf{0.67} & -             \\
% \bottomrule
% \end{tabular}
% }
% \caption{Results for input similarity (larger indicates more similar and better generalization performance)}
% \label{tab:metric_mcqa_input_similarity}
% \end{table}

% \begin{table}[]
% \centering
% \resizebox{0.49\textwidth}{!}{
% \begin{tabular}{llll}
% \toprule
%               & MuTual & DSTC-7 & Ubuntu Dialog \\
% \midrule
% MuTual        & -      & 0.55   & 0.56          \\
% DSTC-7        & 0.56   & -      & 0.56          \\
% Ubuntu Dialog & 0.57   & 0.57   & -            \\
% \bottomrule
% \end{tabular}
% }
% \caption{Results for input similarity (larger indicates more similar and better generalization performance)}
% \label{tab:metric_mcdialog_input_similarity}
% \end{table}


% \begin{table}[]
% \centering
% \resizebox{0.49\textwidth}{!}{
% \begin{tabular}{lllll}
% \toprule
%          & Yelp          & Flipkart      & IMDB       & Amazon     \\
% \midrule
% Yelp     & -             & 0.33          & 1.62       & 1.62       \\
% Flipkart & 0.30          & -             & 0.57       & 0.56       \\
% IMDB     & \textbf{0.25} & 0.29          & -          & \textbf{0} \\
% Amazon   & \textbf{0.25} & \textbf{0.27} & \textbf{0} & -          \\
% \bottomrule
% \end{tabular}
% }
% \caption{Results for label distribution shift (smaller number indicates more similar and better generalization performance)}
% \label{tab:metric_sa_label_shift}
% \end{table}

% \begin{table}[]
% \centering
% \resizebox{0.49\textwidth}{!}{
% \begin{tabular}{llll}
% \toprule
%            & SocialIQA     & PIQA          & OpenbookQA    \\
% \midrule
% SocialIQA  & -             & \textbf{2.44} & \textbf{0.27} \\
% PIQA       & \textbf{0.38} & -             & 0.59          \\
% OpenbookQA & 1.59          & 3.17          & -             \\
% \bottomrule
% \end{tabular}
% }
% \caption{Results for label distribution shift (smaller number indicates more similar and better generalization performance)}
% \label{tab:metric_mcqa_label_shift}
% \end{table}

% \begin{table}[]
% \centering
% \resizebox{0.49\textwidth}{!}{
% \begin{tabular}{llll}
% \toprule
%               & Mutual & DSTC-7 & Ubuntu Dialog \\
% \midrule
% Mutual        & 0      & 0      & 0             \\
% DSTC-7        & 0      & 0      & 0             \\
% Ubuntu Dialog & 0      & 0      & 0             \\
% \bottomrule
% \end{tabular}
% }
% \caption{Results for label distribution shift (smaller number indicates more similar and better generalization performance)}
% \label{tab:metric_mcdialog_label_shift}
% \end{table}


% \begin{table}[]
% \centering
% \resizebox{0.49\textwidth}{!}{
% \begin{tabular}{llll}
% \toprule
%            & SocialIQA     & PIQA          & OpenbookQA    \\
% \midrule
% SocialIQA  & -             & 0.40          & 0.37          \\
% PIQA       & 0.44          & -             & \textbf{0.43} \\
% OpenbookQA & \textbf{0.50} & \textbf{0.54} & -            \\
% \bottomrule
% \end{tabular}
% }
% \caption{Results for input n-gram inclusion (larger number indicates more similar and better generalization performance)}
% \label{tab:metric_mcqa_input_cover}
% \end{table}





% \begin{table}[]
% \begin{tabular}{llll}
% \toprule
%                  & SocialIQA & PIQA & OpenbookQA    \\
% \midrule
% word 1-gram (\%) & 0.43      & 0.51 & \textbf{0.58} \\
% char 4-gram (\%) & 0.50      & 0.60 & \textbf{0.65} \\
% \bottomrule
% \end{tabular}
% \end{table}



% \begin{table}[]
% \begin{tabular}{llll}
% \toprule
%            & SocialIQA     & PIQA          & OpenbookQA    \\
% \midrule
% SocialIQA  & -             & 0.39          & 0.38          \\
% PIQA       & 0.47          & -             & \textbf{0.46} \\
% OpenbookQA & \textbf{0.51} & \textbf{0.52} & \textbf{-}    \\
% \bottomrule
% \end{tabular}
% \end{table}

% \begin{table}[]
% \begin{tabular}{llll}
% \toprule
%            & SocialIQA     & PIQA          & OpenbookQA    \\
% \midrule
% SocialIQA  & -             & 0.51          & 0.51          \\
% PIQA       & 0.60          & -             & \textbf{0.58} \\
% OpenbookQA & \textbf{0.66} & \textbf{0.64} & \textbf{-}    \\
% \bottomrule
% \end{tabular}
% \end{table}


